Efficient Patient Fine-Tuned Seizure Detection with a Tensor Kernel Machine

Recent developments in wearable devices have made accurate and efficient seizure detection more important than ever. A challenge in seizure detection is that patient-specific models typically outperform patient-independent models. However, in a wearable device one typically starts with a patient-independent model, until such patient-specific data is available. To avoid having to construct a new classifier with this data, as required in conventional kernel machines, we propose a transfer learning approach with a tensor kernel machine. This method learns the primal weights in a compressed form using the canonical polyadic decomposition, making it possible to efficiently update the weights of the patient-independent model with patient-specific data. The results show that this patient fine-tuned model reaches as high a performance as a patient-specific SVM model with a model size that is twice as small as the patient-specific model and ten times as small as the patient-independent model.

==> content/discussion.tex <==
\section{Discussion} \label{sec:discussion}
\todo[inline]{
- TL with limited data improves the performance of the seizure classifier\\
- Fewer parameters for T-KRR model 
 - Different transfer learning strategies.\\
 - Investigate an online approach \\
 - Feature selection out of scope \\
 - Using real (behind-the-)ear EEG data
}



% Alternatively, it may just be that we found a better set of hyperparameters for the SVM model, which is potentially due to the fact the T-KRR contains more hyperparameters (i.e. $R$ and $M$). What does speak in favour of the $\text{T-KRR}_{PI}$, is that the model is much smaller (by a factor of 10) than the $\text{SVM}_{PI}$ model, which would make it more suitable for real-time application on a wearable device. \todo{rewrite}

% While the $\text{T-KRR}_{PI}$ classifier may perform slightly worse than its SVM counterpart, it is clear that fine-tuning with patient-specific data results in an improved performance. 

% The results in Figure \ref{fig:boxplot} show that the PI model of the SVM seems to outperform the $\text{T-KRR}_{PI}$ model. 
% This result may be due to the approximation of the Gaussian kernel \eqref{eq:fourier_feat} or the low-rank CPD assumption of the weight tensor. 
% However, while it may be slightly worse performance-wise, the model has much fewer parameters (by a factor of 10) than the SVM model. 
% In future work it may be worth investigating whether a different feature map (e.g. polynomial) could improve the performance of the $\text{T-KRR}_{PI}$ model. 

% In future work, we wish to investigate the effectiveness of the T-KRR classifier for \textit{online} transfer learning, such that a seizure detector could be adapted in real-time. 

